Graph Rewriting for Graph Neural Networks

Given graphs as input, Graph Neural Networks (GNNs) support the inference of nodes, edges, attributes, or graph properties. Graph Rewriting investigates the rule-based manipulation of graphs to model complex graph transformations. We propose that, therefore, (i) graph rewriting subsumes GNNs and could serve as formal model to study and compare them, and (ii) the representation of GNNs as graph rewrite systems can help to design and analyse GNNs, their architectures and algorithms. Hence we propose Graph Rewriting Neural Networks (GReNN) as both novel semantic foundation and engineering discipline for GNNs. We develop a case study reminiscent of a Message Passing Neural Network realised as a Groove graph rewriting model and explore its incremental operation in response to dynamic updates.

==> bibsRH/links.tex <==

\usepackage{html}

\newcommand{\urlink}[1]{\htmladdnormallink{\url{#1}}{#1}} %{\underline{#1}} %
\newcommand{\link}{\htmladdnormallink} %{\underline{#1}}  %

%%% Local People:

\newcommand{\ralph}{\link{Ralph Depke}
{http://www.uni-paderborn.de/cs/ag-engels/ag_dt/People/RalphDepke.html}}

\newcommand{\gregor}{\link{Gregor Engels} 
{http://www.uni-paderborn.de/cs/ag-engels/ag_dt/People/GregorEngels.html}}

\newcommand{\jens}{\link{Jens Gaulke}
{http://www.uni-paderborn.de/cs/ag-engels/ag_dt/People/JensGaulke.html}}

\newcommand{\reiko}{\link{Reiko Heckel}
{http://www.uni-paderborn.de/cs/ag-engels/ag_dt/People/ReikoHeckel.html}}

\newcommand{\jochen}{\link{Jochen K\"uster}
{http://www.uni-paderborn.de/cs/ag-engels/ag_dt/People/JochenKuester.html}}
   
\newcommand{\katharina}{\link{Katharina Mehner}
{http://www.uni-paderborn.de/cs/ag-engels/ag_dt/People/KatharinaMehner.html}}

\newcommand{\stefan}{\link{Stefan Sauer}{http://www.uni-paderborn.de/cs/ag-engels/ag_dt/People/StefanSauer.html}}

\newcommand{\annika}{\link{Annika Wagner}
{http://www.uni-paderborn.de/cs/ag-engels/ag_dt/People/AnnikaWagner.html}}


%%% Remote People: 

\newcommand{\ac}{\link{Andrea Corradini}{http://www.di.unipi.it/~andrea}}
% Andrea Corradini (University of Pisa, Italy)

\newcommand{\um}{\link{Ugo Montanari}{http://www.di.unipi.it/~ugo}}
 % Ugo Montanari (University of Pisa, Italy)

\newcommand{\fg}{\link{Fabio Gadducci}{http://www.di.unipi.it/~gadducci}}
 % Fabio Gadducci (University of Pisa, Italy)

\newcommand{\he}{\link{Hartmut Ehrig}{http://www.cs.tu-berlin.de/~ehrig}}
 % Hartmut Ehrig (Technical University of Berlin, Germany)

\newcommand{\gt}{\link{Gabi Taentzer}{http://www.cs.tu-berlin.de/~gabi}}
 % Gabi Taentzer (Technical University of Berlin, Germany)

\newcommand{\mgr}
{\link{Martin Gro{\ss}e-Rhode}{http://www.cs.tu-berlin.de/~mgr}}
 % Martin Gro{\ss}e-Rhode (Technical University of Berlin, Germany),

\newcommand{\mk}{\link{Manuel Koch}{http://www.cs.tu-berlin.de/~carr}}
 %Manuel Koch (Technical University of Berlin, Germany)

\newcommand{\gb}{\link{Giorgio Busatto}{http://www.wi.leidenuniv.nl/~busatto}}
 % Giorgio Busatto (Leiden University, The Netherlands)

\newcommand{\gr}{\link{Grzegorz Rozenberg}
{http://www.wi.leidenuniv.nl/~rozenber}}
 % Grzegorz Rozenberg (Leiden University, The Netherlands)

\newcommand{\as}{\link{Andy Sch\"urr}{http://inf2-www.informatik.unibw-muenchen.de/People/schuerr}}
 % Andy Sch\"urr (University of the Federal Armed Forces, Munich, Germany)  

\newcommand{\bh}{\link{Berthold Hoffmann}
{http://www.informatik.uni-bremen.de/~hof/}}
 % Berthold Hoffmann and Sabine Kuske (University of Bremen, Germany)

\newcommand{\sk}{\link{Sabine Kuske}
{http://www.informatik.uni-bremen.de/~kuske}}
 % Sabine Kuske (University of Bremen, Germany)

\newcommand{\ml}{\link{Merc\`e Llabr\'es}{http://dmi.uib.es/~merce}}
% Merc\`e Llabr\'es (University of the Balearic Islands, Spain),

\newcommand{\fo}{\link{Fernando Orejas}
{http://orchid.lsi.upc.es:80/~forejas/home.html}}
% Fernando Orejas (Technical University of Catalonia, Spain)


%%% Files 

%\newcommand{\localps}[1]
%{\link{http://www.uni-paderborn.de/cs/ag-engels/Papers/#1.ps.gz}}

\newcommand{\localfile}[1]
{\link{http://www.uni-paderborn.de/cs/ag-engels/Papers/#1}{http://www.uni-paderborn.de/cs/ag-engels/Papers/#1}}

\newcommand{\tfspages}{\link{http://tfs.cs.tu-berlin.de}{http://tfs.cs.tu-berlin.de/publikationen/publications.html}}



